On Overcoming Miscalibrated Conversational Priors in LLM-based Chatbots

We explore the use of Large Language Model (LLM-based) chatbots to power recommender systems. We observe that the chatbots respond poorly when they encounter under-specified requests (e.g., they make incorrect assumptions, hedge with a long response, or refuse to answer). We conjecture that such miscalibrated response tendencies (i.e., conversational priors) can be attributed to LLM fine-tuning using annotators -- single-turn annotations may not capture multi-turn conversation utility, and the annotators' preferences may not even be representative of users interacting with a recommender system. We first analyze public LLM chat logs to conclude that query under-specification is common. Next, we study synthetic recommendation problems with configurable latent item utilities and frame them as Partially Observed Decision Processes (PODP). We find that pre-trained LLMs can be sub-optimal for PODPs and derive better policies that clarify under-specified queries when appropriate. Then, we re-calibrate LLMs by prompting them with learned control messages to approximate the improved policy. Finally, we show empirically that our lightweight learning approach effectively uses logged conversation data to re-calibrate the response strategies of LLM-based chatbots for recommendation tasks.

==> appendices/notation.tex <==
\section{Notation}
\label{sec:notation}
In Table \ref{tab:notation}, we present an overview of the notation used in the paper.
\begin{table}[!htb]
{\renewcommand{\arraystretch}{2}%
	\caption{Notation used in our paper, with notes on interpretation.} \label{tab:notation}
	\resizebox{\textwidth}{!}{\begin{tabular}{|lll|}
	\hline 
        % Queries, copilot responses, and associated attributes
        \multicolumn{3}{|l|}{\textbf{Queries, copilot responses, and associated attributes} explanation here} \\ \hline
        \multicolumn{1}{|l|}{Fully-specified query} 
            & \multicolumn{1}{l|}{
            $\begin{aligned}
            q_f \in Q
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Partially-specified/masked query}
            & \multicolumn{1}{l|}{
            $\begin{aligned}
            q_m \in Q
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Copilot response strategy}             
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            \pi: Q \rightarrow Y
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Copilot response (given $q, \pi$)}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            y \in Y \ | \ q \in Q, \pi \in \Pi
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Minimum viable copilot response}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            
            \end{aligned}$}
            &  test\\ \hline
        % Synthetic query generation
        \multicolumn{3}{|l|}{\textbf{Synthetic query generation} explanation here} \\ \hline
        \multicolumn{1}{|l|}{Intent space}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            \mathcal{I}~\coloneq~\{\text{exercise, gift, movie, plant, travel}\}
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Intent-specific attribute space}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            \Theta_i \coloneq \{\theta_1, \dots, \theta_{|\Theta_i|}\}
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Attribute-specific options}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            X_{\theta \in \Theta_i} \coloneq \{x \ | \ x \text{ is an option for } \theta\}
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Intent-specific query template}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Number of attributes to omit}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            n \sim U(\{1, \dots, |\Theta_i|\})
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Masked attributes}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            \Theta^m_i  \sim U(S_n(\Theta_i))
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Revealed attributes}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            \Theta^r_i \coloneq \Theta_i \setminus \Theta^m_i
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{``Depends on'' attributes}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            
            \end{aligned}$}
            &  test\\ \hline
        % Single-step response evaluation functions
        \multicolumn{3}{|l|}{\textbf{Single-turn response evaluation functions} explanation} \\ \hline
        \multicolumn{1}{|l|}{Utility function}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            \textbf{utility}_{ST}: (q_m, y_\pi) \in Q \times Y_\pi \mapsto \frac{|\phi(y_\pi)|^\gamma}{|q_{\Theta^m_i}|} \in [0,1]
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Cost function}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Cost-aware utility function}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Single-turn oracle policy}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            
            \end{aligned}$}
            &  test\\ \hline

        % Multi-step response evaluation functions
        \multicolumn{3}{|l|}{\textbf{Multi-turn response evaluation functions} explanation here} \\ \hline
        \multicolumn{1}{|l|}{Utility function}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Cost function}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Cost-aware utility function}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            
            \end{aligned}$}
            &  test\\ \hline
        \multicolumn{1}{|l|}{Multi-turn oracle policy}
        & \multicolumn{1}{l|}{
            $\begin{aligned}
            
            \end{aligned}$}
            &  test\\ \hline


	\end{tabular}
 } 
}
\end{table}

==> sections/empirical_eval.tex <==
\section{Empirical Evaluation}
\label{sec:empiricalEvaluation}
In this section, we present results for a set of experiments designed to demonstrate that (1) 
$\defaultPolicy{}$ is miscalibrated in some commonly occurring situations characterized by query underspecification; (2) the approach we propose in Section~\ref{sec:algApproach} is able to recalibrate $\defaultPolicy{}$ to respond more appropriately in the face of underspecification; and (3) our recalibrated meta-policy, $\recalibratedPolicy{}$, results in improved expected reward relative to baseline in the multi-turn recommendation setting.

\subsection{Experimental Setup}
\label{sec:experimentalSetup}

\par \textbf{Datasets}:

\par \textbf{Response strategies}:

\par \textbf{Helper subroutines}:

\par \textbf{Response evaluation functions}


Experiments we conduct to validate the LLM-based operations we perform in the main experiments:
\begin{itemize}
    \item Experiment 0.1 (GPT4): How good is our "detect under-specification" classifer? This is needed because we use this classifier in Experiment 1. Use the "Can LLMs reliably detect under-specification" results, perhaps put in appendix. % use synthetic queries
    \item EXPERIMENT 0.2 (GPT4): How good is our "detect tau" classifer? This is needed because we use this classifier in Experiment 2. Perhaps put in appendix.
    \item EXPERIMENT 0.3 (GPT4): If using LLM as a "User Model", how do we ensure it is not leaking additional information about latent preferences/relevances? This is needed because we use such User Models in Experiment 4,5.
\end{itemize}

\begin{itemize}
    \item EXPERIMENT 1 (GPT4): What fraction of real-world queries are under-specified? --> run the "detect under-specification" setup on a slice of real-world queries (e.g. OpenAssistant dataset).
    \item EXPERIMENT 2 (GPT4):  How controllable is the $\pi_{LLM}$ by switching the prompts for it? Create Figure 4 (histogram of tau's) for $\pi_{LLM}$ responses. Do this also for tau-prompted LLMs. Verify that setting the sys message to tau indeed produces responses of that type w.h.p.
    % 
\end{itemize}

\textcolor{magenta}{I'm going to summarize the setup and drop in summary plots as we get results; text/plots are not final, just an attempt to get all the pieces in place that we can refine when we have a sense of exact narrative}
\par \textbf{Experiment 1 (GPT4): What fraction of real-world queries are under-specified?}

In this experiment, we draw a random subsample of 600 queries from the Open Assistant 1 dataset~\cite{köpf2023openassistant}.  This dataset consists of conversational trees, where levels in the tree correspond to alternating conversational turns between a user and ``assistant''. We are interested in under-specification at $t_0$; as such, we restrict our attention to the root nodes of each conversational tree, as these nodes contain the first user-issued utterance. Additional inclusion criteria include: queries should be classified as English language, and contain at least 3 (not necessarily unique) unigrams. We then ask a helper LLM (GPT4) to review each query $q \in C_{\text{oasst}}$ and map it to exactly one predicted label, $\hat{y}$. The prompt for this task describes and distinguishes between the labels as follows (see Appendix \ref{app:meOneClassify} for details):
\begin{itemize}[left=0pt]
    \item \textsc{sufficient}: All important factors upon which an answer to this query might depend are sufficiently specified.
    \item \textsc{Minor under}: One or more less important factors upon which an answer to this query might depend are not specified or are unknown; however, it is possible to provide a high-quality response even without knowing these factors.
    \item \textsc{Critical under}: One or more important factors upon which an answer to this query might depend are not specified or are unknown; it is difficult to provide a high-quality response without knowing these factors.
\end{itemize}


\par \textbf{Experiment 2 (GPT4):  How controllable is $\pi_{LLM}$ when we condition on different $\tau \in \mathcal{T}$}
In this experiment, we take our synthetic query corpus and ask each LLM that we evaluate (currently, GPT4) to generate a set of responses, where each response is conditioned on a different $\tau \in \mathcal{T}$. We then provide a helper LLM (GPT4) with each (query, tau-induced response) pair and ask it to map the response to a label $\hat{\tau} \in \mathcal{T}^\prime$ where  $\mathcal{T}^\prime \coloneq (\mathcal{T} \setminus \{ \text{baseline}\}) \cup \{\text{direct response}\}$. 

\subsection{Does intervention to promote uncertainty reduction improve performance on downstream tasks?}



Options:

Revisit Expt 2.
\begin{itemize}
\item 2-step experiment with masked queries. Utility = if eventual recommended item satisfies fully-specified user preferences.
\end{itemize}

Real-world data.
\begin{itemize}
\item Need a dataset/candidate set that has not already been ingested into LLM, but can fit into context window.
\item Some degree of redundancy / overlap between candidate items
\item Realistic query distribution. Ideas to generate
\begin{itemize}
    \item Use referring search queries for web pages (e.g., what did people search for to get this page?)
    \item Pick a target item and then generate initial queries backwards through LLM instructions
\end{itemize}
\item Algorithm:
\begin{enumerate}
\item Issue (first) query, let system respond.
\item If target item is in output, stop. Else answer question via user model who can only answer general questions about target article, not idiosyncratic things. 
\item Repeat above two steps with max of $K$ rounds. Utility is number of questions asked + number of incorrect items returned before correct one.
\end{enumerate}
\end{itemize}



==> tables/motExp1_tables.tex <==

Overall 
\begin{table}
\label{overall multi-class old}
\begin{tabular}{lllll}
\toprule
 & precision & recall & f1-score & support \\
\midrule
critical\_under & 0.789 & 0.480 & 0.597 & 202 \\
minor\_under & 0.557 & 0.518 & 0.536 & 398 \\
sufficient & 0.758 & 0.893 & 0.820 & 600 \\
accuracy &  &  & 0.699 & 1200 \\
macro avg & 0.701 & 0.630 & 0.651 & 1200 \\
weighted avg & 0.696 & 0.699 & 0.689 & 1200 \\
\bottomrule
\end{tabular}
\caption{overall}
\end{table}
